Politeness Transfer: A Tag and Generate Approach

This paper introduces a new task of politeness transfer which involves converting non-polite sentences to polite sentences while preserving the meaning. We also provide a dataset of more than 1.39 instances automatically labeled for politeness to encourage benchmark evaluations on this new task. We design a tag and generate pipeline that identifies stylistic attributes and subsequently generates a sentence in the target style while preserving most of the source content. For politeness as well as five other transfer tasks, our model outperforms the state-of-the-art methods on automatic metrics for content preservation, with a comparable or better performance on style transfer accuracy. Additionally, our model surpasses existing methods on human evaluations for grammaticality, meaning preservation and transfer accuracy across all the six style transfer tasks. The data and code is located at https://github.com/tag-and-generate.

==> additional_trash.tex <==
% \if 0
% In this work, we present a novel text attribute transfer system that performs effective attribute transfer while making minimal changes to the input. Unlike recent style transfer systems, we don't rely on adversarial losses to train our model. Instead, we rely on the key intuition that most attribute transfer tasks require us to perform slight changes to certain parts of the sentences, while retaining most of the information. Further, the changes do not always involve deletion or addition, and may require either and or both the operations. Our system consists of two seq2seq systems, the first one of which is called marker and the other one is called the filler. The marker learns to add markers at locations it thinks need to be changed to perform attribute transfer. These markers may substitute existing words or may serve as a placeholder for adding new words. The filler takes these markers and adds attribute words that finally move the input sentence to the desired attribute. Our system is able to improve on or match the performance on all the existing datasets as given by attribute classifiers, and surpasses all the existing systems on content-preserving metrics by a large margin.

% The goal of our system is to transfer a source sentence into a given style attribute.  While most of the common examples in the literature focus on datasets that go from one attribute to another, another common case where the style transfer has to happen from a source sentence that does not have a specific attribute has received little attention. To this end, we present a new task of politeness transfer the corresponding dataset. Additionally, we evaluate our system on the other widely accepted attribute transfer datasets.

% In order to underscore our model's ability to handle the case of add only changes, we needed a dataset that would have a well defined target attribute class but a fuzzy or ill-defined notion of the other class. While looking for such datasets, not only did we realize that such a dataset does not exist, but we also discovered that the community at large has been focused on attribute transfer for cases wherein both the extremes are well defined. 

% Typical examples include performing attribute transfer on sentiment  (positive vs negative), political narrative (democratic vs republican), gender (male vs female) and the likes. However, these bi-modal cases leave out an important class of attribute transfer that are prevalent in everyday discourse: the cases where the attribute is well defined but it's complement is either not well defined or encompasses everything else (one vs. all). We identify examples of two such kinds of text attributes: racism and politeness. In both the cases, while it is relatively easy to identify and define the examples that have the attribute (racist/polite text), the definition of the complementary set is basically just that: ``not-racist'' and ``not-polite''. Note that we don't focus on cases where the sentence has a curse word and is thus impolite, because they would form non-interesting and trivial examples (and can typically be brought to the neutral zone by a mere deletion of curse words). In order to evaluate our systems on such instances and to bring the attention of the community at large, we curate and release a politeness transfer dataset, derived from the Enron email corpus \cite{klimt2004introducing}.


% To compare our work with the state-of-the-art  approaches  of  style  transfer  for  non-parallel  corpus  we  perform  gender transfer, political slant transfer and sentiment  transfer, replicating the models and experimental setups of \cite{shen2017style}, \cite{prabhumoye-etal-2018-style} and \cite{li-etal-2018-delete}.

% \sm{1. What is politeness, how is it relevant in social interactions, applications \\
% 2. limitations and problems with current methods: content transfer. motivation for our model.\\
% 3. our approach and how we overcome the limitations.\\
% 4. politeness : novel, hard overcome\\
% 5. contributions\\
% 2. applications in which style transfer is used 
% \cite{chandu2019my}, dongyeop story telling dataset.}
% \fi


\if 0
\section{Introduction}
Requests are an important part of everyday human exchange. Further, common courtesy typically demands that the requests be polite. While in-person communication can benefit from non-verbal clues like body language, tone and mannerisms to convey politeness, text exchange has to depend entirely on the choice of words and phrasing to convey a request without sounding too imposing. While a bulk of polite requests are made up of words that explicate the intent of the speaker to be polite by using words like  ``please'' and ``thanks'',  the tail consists of a large number of subtle cues, including but not restricted to words and phrases that intend to indicate the speaker's desire to get the request fulfilled without sounding too imposing on the other party. 

A natural question to ask then is what exactly is a polite request? Clearly, the right answer depends on the culture, language, background and social structure of both the speaker and the addressed person. For practical purposes, we restrict our attention to the notion of politeness as widely accepted between the English speakers in a formal setting in north America. For a linguistically motivated definition, we refer the readers to the (). We focus on a complementary, data-driven definition of politeness as given by (). 

In this work, we set to make progress towards the question ``can we take a request and make it more polite?''. The challenges in tackling such a question are manifold. First, we leverage the data-driven definition of politeness as proposed () to draw a boundary around our definition of politeness. Next, we process a dataset of emails to create a setup that can allow us to show the efficacy of our approach on real world datasets. Like most other style transfer problems, since there is no training data present, and the clues for politeness are subtle and unipolar, we propose a novel system that breaks down the problem of controlled text generation into two parts: a) Our first system, the marker, generates politeness markers that identify locations in the text that can be altered. b) The generators takes cues from the markers and learns to recreate a given sentence to make it more polite. 

Most of the current style transfer techniques tackle the problem of transferring text from one extreme distribution to the other. Prevalent popular examples in the literature include transferring sentiment, gender or political opinion. For each of these examples, the boundaries of each of the classes is relatively well defined. However, in certain cases, like politeness, such extremes are either trivially defined or have a fuzzy boundary. Furthermore, it might not be meaningful to go from the well defined class to the trivial extreme. Consider the example ``send me the data". This sentence is not polite, however, at the same time, it is not impolite. Consider a variant, ``please send me the data", which will be widely accepted to be more polite. We define such class of problems as ``unipolar style transfer".


Our main contributions are as follows:
\begin{itemize}
    \item To the best of our knowledge, no one has presented the problem of poli We release a dataset that contains politeness annotations.
    \item We present politeness as a problem of attribute transfer. 
    \item We highlight the unimodality of politeness; while highlighting something as being polite is easier, the absence of politeness is not necessarily a proof of impolitness. This is in stark contrast with the standard style transfer tasks addressed by the community, in which the distinction is obvious (positive/negative, male/female)
    \item For an email, not every sentence has to be made equally polite. Thus, we need a way to decide the politeness level? [May be something from context?] 
    \item Survey/critic on why regular sentence level style transfers don't work for politeness [and why we choose a delete retrieve based approach.]
    \item Finally we provide a framework which will serve as a baseline for document level politeness transfer.
\end{itemize}

\section{Task Description}
\textbf{4 paragraphs} Talk about what is politeness, talk about what kinds of sentences can be made more polite, why are we focusing on it?, what is the proposed input/output?

\paragraph{Task}
We consider the problem of making a request more polite. For example, given a sentence like ``call me now'', we aim to convert it to a form that would be considered more polite by the addressed person. For this particular case, we aim to transfer the given sentence to something like ``please call me now'' or ``could you please call me now?''.

\paragraph{On uni-polarity of politeness}
Most of the current style transfer techniques tackle the problem of transferring text from one extreme distribution to the other. Prevalent popular examples in the literature include transferring sentiment, gender or political opinion. For each of these examples, the boundaries of each of the classes is relatively well defined. However, in certain cases, like politeness, such extremes are either trivially defined or have a fuzzy boundary. Furthermore, it might not be meaningful to go from the well defined class to the trivial extreme. Consider the example "send me the data". This sentence is not polite, however, at the same time, it is not impolite. Consider a variant, "please send me the data", which will be widely accepted to be more polite. We define such class of problems as ``unipolar style transfer".

\section{A critique of the existing evaluation methods for style transfer}
While it has been long known that automatic metrics are not a very good way of evaluating the performance of NLP systems. During the course of our project, we found that automatic metrics are especially non-informative for politeness transfer. For instance, a system that changes the input sentence by adding a "thank you" in the front would get a very high score on the automatic metrics (BLEU, classifier score). However, from the perspective of achieving the stated goal, such a sentence would be pretty much useless. Thus, just relying on metrics that rely on the surface form or a particular aspect of the system can be extremely misleading. We thus stress that it is very important to not only look at a single automatic metric to evaluate the performance of such systems.

\section{Models}
The masker-unmasker model. Variants:

\begin{itemize}
    \item \textbf{RandomMask $\rightarrow$ Unmask}
    \item \textbf{GMASK $\rightarrow$ Unmask}
    \item \textbf{GMSAK-POS $\rightarrow$ Unmask}
    \item \textbf{GMASK-POS $\rightarrow$ SOFT-BEAM $\rightarrow$ UNMASK}
\end{itemize}
\label{models}


\section{Dataset}

\begin{table}
\centering
\begin{tabular}{llll}
Dataset Name & Style/Attribute                                                                                & Counts - 0 & Counts - 1  \\
Yelp         & \begin{tabular}[c]{@{}l@{}}Sentiment\\\textless{}\textgreater{}(Pos - 1, Neg - 0)\end{tabular} &            &             \\
Amazon       & Sentiment                                                                                      &            &             \\
Enron        & \begin{tabular}[c]{@{}l@{}}Politeness\\\textless{}\textgreater{}(Polite - 1)\end{tabular}      & -          &             \\
             & Gender                                                                                         &            &             \\
             & Political Stance                                                                               &            &             \\
GYAFC        & Formality                                                                                      &            &            
\end{tabular}
\end{table}

\section{Experiments and Results}
\label{sec:length}
evaluation metrics
\input{quantres.tex}

\subsection{Analysis}

% \begin{table}[!htb]
%     \centering
%     \footnotesize
%     \setlength\tabcolsep{4pt}
%     \begin{tabular}{|c|c|c|c|c|c|}\hline
% Model        &       BLEU     &  ROUGE    &   METEOR  &  \thead{Politeness \\ Score} & \thead{Pol \\ Acc} \\ \hline
% DRG-D       &  12.75        &     44.67          &   21.38     &    0.91    &    99.16 \% \\ \hline
% DRG-DR      &   10.63    &     44.96        &   19.96     &      0.8134  &   87.5\% \\ \hline
% \thead{Back \\ Translate}       &        &      &    &     &    \\\hline
% Shen       &        &      &    &    &   \\\hline
% Ours      &     52.53   &    82.7     &  45.35    &   0.6667      &   82.64\%    \\\hline
%     \end{tabular}
%     \caption{\centering{Comparison of our model with popular style transfer methods.}}
%     \label{tab:my_label}
% \end{table}

\section{Related Work}


\section{Conclusion and Future Work}

Some other very important indicators of politeness are casing and punctuation. We don't consider such factors, and focus our attention to the politeness phenomenon induced by words for the following reasons: a) Lack of relevant dataset, b) The lack that such factors play a less important role in the formal communication that we focus on, c) the fact that the effect of casing and punctuation on politeness can be a function the local culture. We leave the exploration of other such clues of politeness for transfer as an important future work.

\bibliography{ref}
\bibliographystyle{acl_natbib}


\newpage

% \nocite{*}

\appendix
\begin{itemize}
    \item We motivate it from a perspective of making email writing easier for people,. Politeness is one aspect which is common when they write an email.
    \item Why different? 1) Nobody has worked on politeness. 
    \item Politeness is a difficult style to transfer. We are working on the domain of emails. Enron data is labelled by a politeness classifier.  
    \item No specific domain.
    \item Unipolar. 
    \item Every sentence can't be made polite.
    \item Knowing when a sentence can me made more polite (and by what degree) is an interesting task by itself.
    \item We don't need delete, retrieve or generate. In fact, our system needs to know when to just add, when to delete, and when to let a sentence flow as is (i.e. without any stylistic transfer).
    \item We are learning the notion of politness from a domain and transferring it to the second domain
\end{itemize}
\fi

==> instructions.tex <==


\section{Experiments}
\label{sec:length}

The conference encourages the submission of additional material that is relevant to the reviewers but not an integral part of the paper.
There are two such types of material: appendices, which can be read, and non-readable supplementary materials, often data or code.
Additional material must be submitted as separate files, and must adhere to the same anonymity guidelines as the main paper.
The paper must be self-contained: it is optional for reviewers to look at the supplementary material.
Papers should not refer, for further detail, to documents, code or data resources that are not available to the reviewers.
Refer to Appendices~\ref{sec:appendix} and \ref{sec:supplemental} for further information. 

Workshop chairs may have different rules for allowed length and whether supplemental material is welcome.
As always, the respective call for papers is the authoritative source.


\section{Anonymity}
As reviewing will be double-blind, papers submitted for review should not include any author information (such as names or affiliations). Furthermore, self-references that reveal the author's identity, \emph{e.g.},
\begin{quote}
We previously showed \citep{Gusfield:97} \ldots
\end{quote}
should be avoided. Instead, use citations such as 
\begin{quote}
\citet{Gusfield:97} previously showed\ldots
\end{quote}
Please do not use anonymous citations and do not include acknowledgements.
\textbf{Papers that do not conform to these requirements may be rejected without review.}

Any preliminary non-archival versions of submitted papers should be listed in the submission form but not in the review version of the paper.
Reviewers are generally aware that authors may present preliminary versions of their work in other venues, but will not be provided the list of previous presentations from the submission form.

Once a paper has been accepted to the conference, the camera-ready version of the paper should include the author's names and affiliations, and is allowed to use self-references.

\paragraph{\LaTeX-specific details:}
For an anonymized submission, ensure that {\small\verb|\aclfinalcopy|} at the top of this document is commented out, and that you have filled in the paper ID number (assigned during the submission process on softconf) where {\small\verb|***|} appears in the {\small\verb|\def\aclpaperid{***}|} definition at the top of this document.
For a camera-ready submission, ensure that {\small\verb|\aclfinalcopy|} at the top of this document is not commented out.


\section{Multiple Submission Policy}
Papers that have been or will be submitted to other meetings or publications must indicate this at submission time in the START submission form, and must be withdrawn from the other venues if accepted by ACL 2020. Authors of papers accepted for presentation at ACL 2020 must notify the program chairs by the camera-ready deadline as to whether the paper will be presented. We will not accept for publication or presentation the papers that overlap significantly in content or results with papers that will be (or have been) published elsewhere.

Authors submitting more than one paper to ACL 2020 must ensure that submissions do not overlap significantly (>25\%) with each other in content or results.



\section{Formatting Instructions}

Manuscripts must be in two-column format.
Exceptions to the two-column format include the title, authors' names and complete addresses, which must be centered at the top of the first page, and any full-width figures or tables (see the guidelines in Section~\ref{ssec:title-authors}).
\textbf{Type single-spaced.}
Start all pages directly under the top margin.
The manuscript should be printed single-sided and its length should not exceed the maximum page limit described in Section~\ref{sec:length}.
Pages should be numbered in the version submitted for review, but \textbf{pages should not be numbered in the camera-ready version}.

\paragraph{\LaTeX-specific details:}
The style files will generate page numbers when {\small\verb|\aclfinalcopy|} is commented out, and remove them otherwise.


\subsection{File Format}
\label{sect:pdf}

For the production of the electronic manuscript you must use Adobe's Portable Document Format (PDF).
Please make sure that your PDF file includes all the necessary fonts (especially tree diagrams, symbols, and fonts with Asian characters).
When you print or create the PDF file, there is usually an option in your printer setup to include none, all or just non-standard fonts.
Please make sure that you select the option of including ALL the fonts.
\textbf{Before sending it, test your PDF by printing it from a computer different from the one where it was created.}
Moreover, some word processors may generate very large PDF files, where each page is rendered as an image.
Such images may reproduce poorly.
In this case, try alternative ways to obtain the PDF.
One way on some systems is to install a driver for a postscript printer, send your document to the printer specifying ``Output to a file'', then convert the file to PDF.

It is of utmost importance to specify the \textbf{A4 format} (21 cm x 29.7 cm) when formatting the paper.
Print-outs of the PDF file on A4 paper should be identical to the hardcopy version.
If you cannot meet the above requirements about the production of your electronic submission, please contact the publication chairs as soon as possible.

\paragraph{\LaTeX-specific details:}
PDF files are usually produced from \LaTeX{} using the \texttt{\small pdflatex} command.
If your version of \LaTeX{} produces Postscript files, \texttt{\small ps2pdf} or \texttt{\small dvipdf} can convert these to PDF.
To ensure A4 format in \LaTeX, use the command {\small\verb|\special{papersize=210mm,297mm}|}
in the \LaTeX{} preamble (below the {\small\verb|\usepackage|} commands) and use \texttt{\small dvipdf} and/or \texttt{\small pdflatex}; or specify \texttt{\small -t a4} when working with \texttt{\small dvips}.

\subsection{Layout}
\label{ssec:layout}

Format manuscripts two columns to a page, in the manner these
instructions are formatted.
The exact dimensions for a page on A4 paper are:

\begin{itemize}
\item Left and right margins: 2.5 cm
\item Top margin: 2.5 cm
\item Bottom margin: 2.5 cm
\item Column width: 7.7 cm
\item Column height: 24.7 cm
\item Gap between columns: 0.6 cm
\end{itemize}

\noindent Papers should not be submitted on any other paper size.
If you cannot meet the above requirements about the production of your electronic submission, please contact the publication chairs above as soon as possible.

\subsection{Fonts}

For reasons of uniformity, Adobe's \textbf{Times Roman} font should be used.
If Times Roman is unavailable, you may use Times New Roman or \textbf{Computer Modern Roman}.

Table~\ref{font-table} specifies what font sizes and styles must be used for each type of text in the manuscript.

\begin{table}
\centering
\begin{tabular}{lrl}
\hline \textbf{Type of Text} & \textbf{Font Size} & \textbf{Style} \\ \hline
paper title & 15 pt & bold \\
author names & 12 pt & bold \\
author affiliation & 12 pt & \\
the word ``Abstract'' & 12 pt & bold \\
section titles & 12 pt & bold \\
subsection titles & 11 pt & bold \\
document text & 11 pt  &\\
captions & 10 pt & \\
abstract text & 10 pt & \\
bibliography & 10 pt & \\
footnotes & 9 pt & \\
\hline
\end{tabular}
\caption{\label{font-table} Font guide. }
\end{table}

\paragraph{\LaTeX-specific details:}
To use Times Roman in \LaTeX2e{}, put the following in the preamble:
\begin{quote}
\small
\begin{verbatim}
\usepackage{times}
\usepackage{latexsym}
\end{verbatim}
\end{quote}


\subsection{Ruler}
A printed ruler (line numbers in the left and right margins of the article) should be presented in the version submitted for review, so that reviewers may comment on particular lines in the paper without circumlocution.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera ready copy should not contain a ruler.

\paragraph{Reviewers:}
note that the ruler measurements may not align well with lines in the paper -- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
In most cases one would expect that the approximate location will be adequate, although you can also use fractional references (\emph{e.g.}, this line ends at mark $295.5$).

\paragraph{\LaTeX-specific details:}
The style files will generate the ruler when {\small\verb|\aclfinalcopy|} is commented out, and remove it otherwise.

\subsection{Title and Authors}
\label{ssec:title-authors}

Center the title, author's name(s) and affiliation(s) across both columns.
Do not use footnotes for affiliations.
Place the title centered at the top of the first page, in a 15-point bold font.
Long titles should be typed on two lines without a blank line intervening.
Put the title 2.5 cm from the top of the page, followed by a blank line, then the author's names(s), and the affiliation on the following line.
Do not use only initials for given names (middle initials are allowed).
Do not format surnames in all capitals (\emph{e.g.}, use ``Mitchell'' not ``MITCHELL'').
Do not format title and section headings in all capitals except for proper names (such as ``BLEU'') that are
conventionally in all capitals.
The affiliation should contain the author's complete address, and if possible, an electronic mail address.

The title, author names and addresses should be completely identical to those entered to the electronical paper submission website in order to maintain the consistency of author information among all publications of the conference.
If they are different, the publication chairs may resolve the difference without consulting with you; so it is in your own interest to double-check that the information is consistent.

Start the body of the first page 7.5 cm from the top of the page.
\textbf{Even in the anonymous version of the paper, you should maintain space for names and addresses so that they will fit in the final (accepted) version.}


\subsection{Abstract}
Use two-column format when you begin the abstract.
Type the abstract at the beginning of the first column.
The width of the abstract text should be smaller than the
width of the columns for the text in the body of the paper by 0.6 cm on each side.
Center the word \textbf{Abstract} in a 12 point bold font above the body of the abstract.
The abstract should be a concise summary of the general thesis and conclusions of the paper.
It should be no longer than 200 words.
The abstract text should be in 10 point font.

\subsection{Text}
Begin typing the main body of the text immediately after the abstract, observing the two-column format as shown in the present document.

Indent 0.4 cm when starting a new paragraph.

\subsection{Sections}

Format section and subsection headings in the style shown on the present document.
Use numbered sections (Arabic numerals) to facilitate cross references.
Number subsections with the section number and the subsection number separated by a dot, in Arabic numerals.

\subsection{Footnotes}
Put footnotes at the bottom of the page and use 9 point font.
They may be numbered or referred to by asterisks or other symbols.\footnote{This is how a footnote should appear.}
Footnotes should be separated from the text by a line.\footnote{Note the line separating the footnotes from the text.}

\subsection{Graphics}

Place figures, tables, and photographs in the paper near where they are first discussed, rather than at the end, if possible.
Wide illustrations may run across both columns.
Color is allowed, but adhere to Section~\ref{ssec:accessibility}'s guidelines on accessibility.

\paragraph{Captions:}
Provide a caption for every illustration; number each one sequentially in the form:
``Figure 1. Caption of the Figure.''
``Table 1. Caption of the Table.''
Type the captions of the figures and tables below the body, using 10 point text.
Captions should be placed below illustrations.
Captions that are one line are centered (see Table~\ref{font-table}).
Captions longer than one line are left-aligned (see Table~\ref{tab:accents}).

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, \BibTeX\ names.}\label{tab:accents}
\end{table}

\paragraph{\LaTeX-specific details:}
The style files are compatible with the caption and subcaption packages; do not add optional arguments.
\textbf{Do not override the default caption sizes.}


\subsection{Hyperlinks}
Within-document and external hyperlinks are indicated with Dark Blue text, Color Hex \#000099.

\subsection{Citations}
Citations within the text appear in parentheses as~\citep{Gusfield:97} or, if the author's name appears in the text itself, as \citet{Gusfield:97}.
Append lowercase letters to the year in cases of ambiguities.  
Treat double authors as in~\citep{Aho:72}, but write as in~\citep{Chandra:81} when more than two authors are involved. Collapse multiple citations as in~\citep{Gusfield:97,Aho:72}. 

Refrain from using full citations as sentence constituents.
Instead of
\begin{quote}
  ``\citep{Gusfield:97} showed that ...''
\end{quote}
write
\begin{quote}
``\citet{Gusfield:97} showed that ...''
\end{quote}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \small\verb|\citep| & \small\verb|\cite| \\
\citealp{Gusfield:97} & \small\verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \small\verb|\citet| & \small\verb|\newcite| \\
\citeyearpar{Gusfield:97} & \small\verb|\citeyearpar| & \small\verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

\paragraph{\LaTeX-specific details:}
Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command {\small\verb|\citet|} (cite in text) to get ``author (year)'' citations as in \citet{Gusfield:97}.
You can use the command {\small\verb|\citep|} (cite in parentheses) to get ``(author, year)'' citations as in \citep{Gusfield:97}.
You can use the command {\small\verb|\citealp|} (alternative cite without  parentheses) to get ``author year'' citations (which is useful for  using citations within parentheses, as in \citealp{Gusfield:97}).


\subsection{References}
Gather the full set of references together under the heading \textbf{References}; place the section before any Appendices. 
Arrange the references alphabetically by first author, rather than by order of occurrence in the text.

Provide as complete a citation as possible, using a consistent format, such as the one for \emph{Computational Linguistics\/} or the one in the  \emph{Publication Manual of the American 
Psychological Association\/}~\citep{APA:83}.
Use full names for authors, not just initials.

Submissions should accurately reference prior and related work, including code and data.
If a piece of prior work appeared in multiple venues, the version that appeared in a refereed, archival venue should be referenced.
If multiple versions of a piece of prior work exist, the one used by the authors should be referenced.
Authors should not rely on automated citation indices to provide accurate references for prior and related work.

The following text cites various types of articles so that the references section of the present document will include them.
\begin{itemize}
\item Example article in journal: \citep{Ando2005}.
\item Example article in proceedings, with location: \citep{borschinger-johnson-2011-particle}.
\item Example article in proceedings, without location: \citep{andrew2007scalable}.
\item Example arxiv paper: \citep{rasooli-tetrault-2015}. 
\end{itemize}


\paragraph{\LaTeX-specific details:}
The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{\small acl2020.bib}, then placing the following before any appendices in your \LaTeX{}  file will generate the references section for you:
\begin{quote}\small
\verb|\bibliographystyle{acl_natbib}|\\
\verb|\bibliography{acl2020}|
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX\ file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the anthology and your own bib file, use the following instead of the above.
\begin{quote}\small
\verb|\bibliographystyle{acl_natbib}|\\
\verb|\bibliography{anthology,acl2020}|
\end{quote}


\subsection{Digital Object Identifiers}
As part of our work to make ACL materials more widely used and cited outside of our discipline, ACL has registered as a CrossRef member, as a registrant of Digital Object Identifiers (DOIs), the standard for registering permanent URNs for referencing scholarly materials.

All camera-ready references are required to contain the appropriate DOIs (or as a second resort, the hyperlinked ACL Anthology Identifier) to all cited works.
Appropriate records should be found for most materials in the current ACL Anthology at \url{http://aclanthology.info/}.
As examples, we cite \citep{goodman-etal-2016-noise} to show you how papers with a DOI will appear in the bibliography.
We cite \citep{harper-2014-learning} to show how papers without a DOI but with an ACL Anthology Identifier will appear in the bibliography.

\paragraph{\LaTeX-specific details:}
Please ensure that you use Bib\TeX\ records that contain DOI or URLs for any of the ACL materials that you reference.
If the Bib\TeX{} file contains DOI fields, the paper title in the references section will appear as a hyperlink to the DOI, using the hyperref \LaTeX{} package.


\subsection{Appendices}
Appendices, if any, directly follow the text and the
references (but only in the camera-ready; see Appendix~\ref{sec:appendix}).
Letter them in sequence and provide an informative title:
\textbf{Appendix A. Title of Appendix}.

\section{Accessibility}
\label{ssec:accessibility}

In an effort to accommodate people who are color-blind (as well as those printing to paper), grayscale readability is strongly encouraged.
Color is not forbidden, but authors should ensure that tables and figures do not rely solely on color to convey critical distinctions.
A simple criterion:
All curves and points in your figures should be clearly distinguishable without color.

\section{Translation of non-English Terms}

It is also advised to supplement non-English characters and terms with appropriate transliterations and/or translations since not all readers understand all such characters and terms.
Inline transliteration or translation can be represented in the order of:
\begin{center}
\begin{tabular}{c}
original-form \\
transliteration \\
``translation''
\end{tabular}
\end{center}

\section{\LaTeX{} Compilation Issues}
You may encounter the following error during compilation: 
\begin{quote}
{\small\verb|\pdfendlink|} ended up in different nesting level than {\small\verb|\pdfstartlink|}.
\end{quote}
This happens when \texttt{\small pdflatex} is used and a citation splits across a page boundary.
To fix this, the style file contains a patch consisting of two lines:
(1) {\small\verb|\RequirePackage{etoolbox}|} (line 455 in \texttt{\small acl2020.sty}), and
(2) A long line below (line 456 in \texttt{\small acl2020.sty}).

If you still encounter compilation issues even with the patch enabled, disable the patch by commenting the two lines, and then disable the \texttt{\small hyperref} package by loading the style file with the \texttt{\small nohyperref} option:

\noindent
{\small\verb|\usepackage[nohyperref]{acl2020}|}

\noindent
Then recompile, find the problematic citation, and rewrite the sentence containing the citation. (See, {\em e.g.}, \url{http://tug.org/errors.html})

\section*{Acknowledgments}

The acknowledgments should go immediately before the references. Do not number the acknowledgments section.
Do not include this section when submitting your paper for review.

\bibliography{anthology,acl2020}
\bibliographystyle{acl_natbib}

\appendix

\section{Appendices}
\label{sec:appendix}
Appendices are material that can be read, and include lemmas, formulas, proofs, and tables that are not critical to the reading and understanding of the paper. 
Appendices should be \textbf{uploaded as supplementary material} when submitting the paper for review.
Upon acceptance, the appendices come after the references, as shown here.

\paragraph{\LaTeX-specific details:}
Use {\small\verb|\appendix|} before any appendix section to switch the section numbering over to letters.


\section{Supplemental Material}
\label{sec:supplemental}
Submissions may include non-readable supplementary material used in the work and described in the paper.
Any accompanying software and/or data should include licenses and documentation of research review as appropriate.
Supplementary material may report preprocessing decisions, model parameters, and other details necessary for the replication of the experiments reported in the paper.
Seemingly small preprocessing decisions can sometimes make a large difference in performance, so it is crucial to record such decisions to precisely characterize state-of-the-art methods. 

Nonetheless, supplementary material should be supplementary (rather than central) to the paper.
\textbf{Submissions that misuse the supplementary material may be rejected without review.}
Supplementary material may include explanations or details of proofs or derivations that do not fit into the paper, lists of
features or feature templates, sample inputs and outputs for a system, pseudo-code or source code, and data.
(Source code and data should be separate uploads, rather than part of the paper).

The paper should not rely on the supplementary material: while the paper may refer to and cite the supplementary material and the supplementary material will be available to the reviewers, they will not be asked to review the supplementary material.


==> qualres.tex <==
% \begin{table*}[!h]
% \centering
% \tiny{
% \begin{tabular}{p{1.6in}@{\hskip 0.1in} p{1.6in}@{\hskip 0.1in}p{1.6in}@{\hskip 0.1in}p{0.75in}} 
% \toprule
% \multicolumn{1}{c}{\textbf{Input}}  & \multicolumn{1}{c}{\textbf{DRG Output}} & \multicolumn{1}{c}{\textbf{Our Model Output}} & \multicolumn{1}{c}{\textbf{Strategy}} \\
% \midrule
% what happened to my personal station? & what happened to my mother to my co??? & \textcolor{green!65!blue}{could you please let me know} what happened to my personal station? & Counterfactual Modal \\
% \addlinespace
% yes, go ahead and remove it. & yes, please go to the link below and delete it. & yes, \textcolor{green!65!blue}{we can} go ahead and remove it. & 1st Person Plural \\
% \addlinespace
% not yet-i'll try this wkend. & not yet to say-i think this will be a \textless{}unk\textgreater{} long. & \textcolor{green!65!blue}{sorry} not yet-i'll try to make sure this wk & Apologizing \\
% \addlinespace
% please check on metromedia energy, & thanks again on the energy industry, & please check on metromedia energy, \textcolor{green!65!blue}{thanks} & Mitigating please start \\
% \midrule
% \end{tabular}}
% \caption{Qualitative Examples comparing the outputs from DRG and Our model for the Politeness Transfer Task}
% \vspace{-0.5em}
% \label{tab:qual_res}
% \end{table*}


% \begin{table*}
% \centering
% \small{
% \begin{tabular}{p{1.5in}@{\hskip 0.1in}p{1.5in}@{\hskip 0.1in}p{1.5in}|c} 
% \toprule
% \multicolumn{1}{c}{\textbf{Input}}  & \multicolumn{1}{c}{\textbf{DRG Output}} & \multicolumn{1}{c}{\textbf{Our Model Output}} & \multicolumn{1}{c}{\textbf{\thead{Politeness \\ Strategy}}} \\
% \midrule

% what happened to my  & what happened to my mother   & \textcolor{green!65!blue}{could you please let me know}  & Counterfactual  \\
% personal station? &   to my co???     &   what happened to my personal     &  Modal \\
%  &        &   station?    & \\
% \addlinespace
% yes, go ahead and remove it. & yes, please go to the link below and delete it. & yes, \textcolor{green!65!blue}{we can} go ahead and remove it. & \thead {1st Person \\ Plural} \\
% \addlinespace
% not yet -- i'll try this wkend. & not yet to say - i think this will be a \textless{}unk\textgreater{} long. & \textcolor{green!65!blue}{sorry} not yet -- i'll try to make sure this wk & Apologizing \\
% \addlinespace
% please check on metromedia energy, & thanks again on the energy industry, & please check on metromedia energy, \textcolor{green!65!blue}{thanks} & \thead{Mitigating \\ Please Start} \\
% \midrule
% \end{tabular}}
% \caption{Qualitative Examples comparing the outputs from DRG and Our model for the Politeness Transfer Task along with analysis highlighting the corresponding politeness strategy}
% \end{table*}


% \begin{table*}
% \centering
% \small{
% \begin{tabular}{p{1.5in}@{\hskip 0.25in} p{1.5in}@{\hskip 0.25in}p{1.5in}@{\hskip 0.25in}c} 
% \toprule
% \multicolumn{1}{c}{\textbf{Input}}  & \multicolumn{1}{c}{\textbf{DRG Output}} & \multicolumn{1}{c}{\textbf{Our Model Output}} & \multicolumn{1}{c}{\textbf{\thead{Politeness \\ Strategy}}} \\
% \midrule
% what happened to my personal station? & what happened to my mother to my co??? & \textcolor{green!65!blue}{could you please let me know} what happened to my personal station? & \thead{Counterfactual-modal} \\
% \addlinespace
% yes, go ahead and remove it. & yes, please go to the link below and delete it. & yes, \textcolor{green!65!blue}{we can} go ahead and remove it. & 1st Person Plural \\
% \addlinespace
% not yet -- i'll try this wkend. & not yet to say - i think this will be a \textless{}unk\textgreater{} long. & \textcolor{green!65!blue}{sorry} not yet -- i'll try to make sure this wk & Apologizing \\
% \addlinespace
% please check on metromedia energy, & thanks again on the energy industry, & please check on metromedia energy, \textcolor{green!65!blue}{thanks} & Mitigating Please Start \\
% \midrule
% \end{tabular}}
% \caption{Qualitative Examples comparing the outputs from DRG and Our model for the Politeness Transfer Task along with analysis highlighting the corresponding politeness strategy}
% \end{table*}

